CIDOR: Content Distribution and Retrieval in Disaster Networks for Public Protection

Information-Centric Networking (ICN) introduces a paradigm shift from a host centric communication model for Future Internet architectures. It supports the retrieval of a particular content regardless of the physical location of the content. Emergency network in a disaster scenario or disruptive network presents a significant challenge to the ICN deployment. In this paper, we present a Content dIstribution and retrieval framework in disaster netwOrks for public pRotection (CIDOR) which exploits the design principle of the native CCN architecture in the native Delay Tolerant Networking (DTN) architecture. We prove the feasibility and investigate the performance of our proposed solution using extensive simulation with different classes of the DTN routing strategies in different mobility scenarios. The simulation result shows that CIDOR can reduce the content retrieval time up to 50% while the response ratio is close to 100%.

==> intro.tex <==
\section{Introduction}

Today's Internet architecture very much relies on the fundamental assumption that there exists an end-to-end path between the source and destination for the duration of a communication session. Rapid developments and technological advances have enriched the mobile technology with a variety of embedded sensors, such as GPS, camera, and digital compass. Users can create their own content and share it with other people through social networks. Therefore, the vast majority of Internet usage is dominated by the content distribution and retrieval of a large amount of digital content. The conventional Internet is becoming increasingly infeasible and less meaningful in terms of a number of recognized limitations, for instance, decoupling address from an end-point identity, mobility and disruption tolerance, and above all, scalable and efficient content distribution.

In response to these, Information-Centric Networking (ICN) architecture (e.g., CCN \cite{jacobson2009networking}, DONA \cite{koponen2007data}, PURSUIT/PSIRP \cite{tarkoma2009publish}, POINT \cite{point}, NetInf \cite{dannewitz2009netinf}) emerges a paradigm shift from host centric to information centric communication model. It supports the retrieval of a particular content without any reference to the physical location of the content. \textit{Named data} is the central element of ICN communication instead of its physical location. When a node needs content, it sends a request for a particular content. If any node on the way of the request packet has the content in its content store, it replies the content back to the requester.

Intermittently connected network topology or network disruption incurs a significant challenge for ICN deployment. For instance, name resolution may fail due to network disruptions especially when the elements of the distributed resolution services are affected by network partitioning, such as the consequence of a disaster scenario like hurricane, earthquake, or tsunami. Moreover, name resolution may become unreliable, particularly when names are resolved to locator(s) that do not exist anymore. On March 2011, a magnitude-9 earthquake struck northeastern Japan. The power generation systems, fixed infrastructure networks and mobile telephony towers were completely destroyed. The satellite telecommunication equipment was used for relief and rescue activities, as well as to provide emergency humanitarian assistance. Presently, GreenICN EU-Japan project \cite{green} has given effort to exploit the ICN usage in disaster scenario, when it is difficult to efficiently disseminate disaster notifications and critical rescue information. 


In contrast, Delay-tolerant networking (DTN) \cite{cerf2007delay} is an initiative that introduces an architecture for such scenarios, which are particularly characterized by long delay paths, frequent unpredictable disconnections and network partitions. This architecture provides a flexible and resilient protocol for such networks. DTN is based on the store-carry-and-forward model utilizing persistent storage that is well distributed throughout the network. All data are cached in the network until an opportunistic contact is available to forward data. 

The goal of this paper is to design a content-centric architecture in DTN called C2DTN that enriches the connectivity options of the native CCN in disaster scenario. For this, C2DTN implements the content-centric features on top of the Bundle Protocol (BP) \cite{burleigh2007bundle} of DTN architecture. 

In summary, the main contributions of this paper are as follows:
\begin{itemize}
  \item Integration of BP interface to the forwarding scheme of the CCN router \cite{ccnx} (Figure~\ref{c2dtn_node}).
  %\item Introduce Opportunistic Cache (Section~\ref{oc}).  
  \item Extension of the DTN message to support the seamless integration of the Bundle Protocol in the native CCN (Section~\ref{format}).
  \item \textit{Duplicate suppression} and \textit{Redundancy elimination} mechanism at content level (Section~\ref{duplicate} and ~\ref{re}).
  \item Modular design to support the existing DTN routing strategies during the forwarding of messages using BP. 
  \item A thorough evaluation of the efficiency of C2DTN architecture using simulation with different classes of DTN routing strategies for different mobility scenarios.
\end{itemize}

The rest of this paper is organized as follows: We first introduce the background in Section~\ref{back}. Section~\ref{motivation} defines the problem statement and gives an overview of our solution. Section~\ref{design} describes our proposed architecture and the implementation details. After that, the proposed architecture is evaluated in Section~\ref{result}, with different classes of DTN routing strategies for the different mobility scenarios. Section~\ref{related} investigates the related work and finally, Section~\ref{conclude} concludes the paper. 
